Gated3D: Monocular 3D Object Detection From Temporal Illumination Cues

Today's state-of-the-art methods for 3D object detection are based on lidar, stereo, or monocular cameras. Lidar-based methods achieve the best accuracy, but have a large footprint, high cost, and mechanically-limited angular sampling rates, resulting in low spatial resolution at long ranges. Recent approaches based on low-cost monocular or stereo cameras promise to overcome these limitations but struggle in low-light or low-contrast regions as they rely on passive CMOS sensors. In this work, we propose a novel 3D object detection modality that exploits temporal illumination cues from a low-cost monocular gated imager. We propose a novel deep detector architecture, Gated3D, that is tailored to temporal illumination cues from three gated images. Gated images allow us to exploit mature 2D object feature extractors that guide the 3D predictions through a frustum segment estimation. We assess the proposed method on a novel 3D detection dataset that includes gated imagery captured in over 10,000 km of driving data. We validate that our method outperforms state-of-the-art monocular and stereo approaches at long distances. We will release our code and dataset, opening up a new sensor modality as an avenue to replace lidar in autonomous driving.

==> fig/real_dataset_distribution.tex <==
\begin{tikzpicture}
\begin{axis}[
	title=Real Dataset,
	symbolic x coords={clear, snow, fog},
	ylabel=Samples,
	xtick={clear, snow, fog},
	tick label style={/pgf/number format/fixed},
	scaled ticks=false,
	enlarge x limits=0.3,
	legend style={legend columns=-1},
	legend pos=north east,
	ybar=6pt,% configures `bar shift'
	bar width=20pt,
	width=0.98\columnwidth,
	height=0.6\columnwidth,
	ymin=0,
]
\addplot[fill=dai_deepred, dai_deepred] 
	coordinates {(clear,9267) (snow,1516) (fog,848)};

\addplot[fill=dai_petrol, dai_petrol]  
	coordinates {(clear,5010) (snow,788) (fog,257)};

\legend{Day,Night}
\end{axis}
\end{tikzpicture}

==> fig/real_dataset_examples.tex <==
\setlength\tabcolsep{1.5pt}
		\begin{tabular}{cccccc}
		
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-08_17-37-26_00278_rgb.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-08_17-45-07_00027_rgb.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-12_17-03-58_01048_rgb.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-04_10-00-03_00082_rgb.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-04_10-18-44_00322_rgb.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-12_12-10-05_00447_rgb.jpg} \\[2pt]
		
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-08_17-37-26_00278_gated1.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-08_17-45-07_00027_gated1.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-12_17-03-58_01048_gated1.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-04_10-00-03_00082_gated1.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-04_10-18-44_00322_gated1.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-12_12-10-05_00447_gated1.jpg} \\[2pt]
				
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-08_17-37-26_00278_lidar.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-08_17-45-07_00027_lidar.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-12_17-03-58_01048_lidar.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-04_10-00-03_00082_lidar.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-04_10-18-44_00322_lidar.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/real_dataset_examples/2018-02-12_12-10-05_00447_lidar.jpg} \\
					
		\end{tabular}

==> fig/rip_measurements.tex <==
\begin{tikzpicture}
				\begin{axis}
					[
					ylabel=$C_{i}(r)$,
					xmin=10, xmax=100,
					ymin=-100, ymax=1100,
					legend style={
						cells={anchor=west},
						legend pos=north east,
						font=\scriptsize
					},
					legend columns=3, 
					legend entries={$\tilde{C}_1(r)$, $\tilde{C}_2(r)$, $\tilde{C}_3(r)$},
					height=0.38\columnwidth,
					width=\linewidth
					]
				
				\addlegendimage{very thick, densely dashed, dai_deepred}
				\addlegendimage{very thick, densely dashed, dai_petrol}
				\addlegendimage{very thick, densely dashed, dai_ligth_grey40K}
				
				\addplot+ 	[
							thick,
							dai_ligth_grey40K,
							only marks,
							mark=x,
							mark options={color=dai_ligth_grey40K},
							mark size=2.5pt,
							]
				table[x index=0,y index=3,col sep=space]{fig/rip_real.txt};
				
				\addplot+ 	[
							thick,
							dai_petrol,
							only marks,
							mark=x,
							mark options={color=dai_petrol},
							mark size=2.5pt,
							]
				table[x index=0,y index=2,col sep=space]{fig/rip_real.txt};
				
				\addplot+ 	[
							thick,
							dai_deepred,
							only marks,
							mark=x,
							mark options={color=dai_deepred},
							mark size=2.5pt,
							]
				table[x index=0,y index=1,col sep=space]{fig/rip_real.txt};
				
				\addplot+ 	[
							mark=none,
							densely dashed,
							thick, 
							dai_deepred,
							]
				table[x index=0,y index=1, col sep=space]{fig/rip_cheb.txt};
								
				\addplot+ 	[
							mark=none,
							densely dashed,
							thick, 
							dai_petrol,
				]
				table[x index=0,y index=2, col sep=space]{fig/rip_cheb.txt};
								
				\addplot+ 	[
							mark=none,
							densely dashed,
							thick, 
							dai_ligth_grey40K,
							]
				table[x index=0,y index=3, col sep=space]{fig/rip_cheb.txt};
				
				\end{axis}
	\end{tikzpicture}

==> fig/synthetic_dataset_distribution.tex <==
\begin{tikzpicture}
\begin{axis}[
	title=Synthetic Dataset,
    symbolic x coords={urban, highway, overland},
	xtick={urban, highway, overland},
	enlarge x limits=0.3,
	legend style={legend columns=-1},
	legend pos=north east,
	ybar=6pt,
	bar width=20pt,
	width=0.98\columnwidth,
	height=0.6\columnwidth,
	ymin=0,
]
\addplot[fill=dai_deepred, dai_deepred] 
	coordinates {(urban,4470) (highway,1061) (overland,862)};

\addplot[fill=dai_petrol, dai_petrol] 
	coordinates {(urban,2201) (highway,593) (overland,617)};

\legend{Day,Night}
\end{axis}
\end{tikzpicture}

==> fig/synthetic_dataset_examples.tex <==
\setlength\tabcolsep{1.5pt}
\begin{tabular}{cccccc}
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0000012456_rgb.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0000175288_rgb.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0000906010_rgb.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0001107339_rgb.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-10_04-25-32_0000121056_rgb.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-10_04-25-32_0000220326_rgb.jpg} \\[2pt]
		
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0000012456_gated1.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0000175288_gated1.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0000906010_gated1.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0001107339_gated1.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-10_04-25-32_0000121056_gated1.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-10_04-25-32_0000220326_gated1.jpg} \\[2pt]
				
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0000012456_lidar.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0000175288_lidar.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0000906010_lidar.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-05_20-02-08_0001107339_lidar.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-10_04-25-32_0000121056_lidar.jpg} &
		\includegraphics[width=0.16\textwidth]{fig/gta_dataset_examples/2018-09-10_04-25-32_0000220326_lidar.jpg} \\
			
		\end{tabular}
